Nonlocal Lagrangian fields and the second Noether theorem. Non-commutative $U(1)$ gauge theory

This article focuses on three main contributions. Firstly, we provide an in-depth overview of the nonlocal Lagrangian formalism. Secondly, we introduce an extended version of the second Noether's theorem tailored for nonlocal Lagrangians. Finally, we apply both the formalism and the extended theorem to the context of non-commutative U(1) gauge theory, including its Hamiltonian and quantization, showcasing their practical utility.

==> NC1-SeibergWitten.tex <==
 \section{The Seiberg-Witten map revisited \label{SW}}
The equation (\ref{AG4}) of Section \ref{S3.1a}, besides being the basis of the algorithm to solve the field equations, can also be read as a correspondence between the nonlocal gauge theory of the $A_a$ field and that of the $Z_a$ field corresponding to a local gauge theory, which is none other than the electromagnetic field. In this section, we will now develop this point of view. 

The field equations (\ref{NC8}) can be written as follows
$$ \psi^c(x) \equiv \mathcal{E}^c_a  A^a + \Lambda^c (A_a) \,,$$
with
\begin{equation}  \label{SWM1}
\mathcal{E}^c_a := \Box \,\delta^c_a - \partial^c \partial_a  \qquad {\rm and} \qquad 
\Lambda^c (A_a) := - i\,\partial_a \left[A^a,A^c\right] - i\,\left[A_a,F^{ac}\right] \,.
\end{equation} 
We then define
\begin{equation}  \label{SWM2}
Z_a := A_a + \Box^{-1} \Lambda_a(A_e) \,,
\end{equation} 
where $\Box^{-1}$ means an elementary solution of the D'Alembert inhomogeneous equation. We easily obtain that
$$ \mathcal{E}^c_a Z^a \equiv \psi^c - \Box^{-1} \partial^c\left(\partial_a \Lambda^a\right) \,. $$
Now, from the identity (\ref{NC13}) and the fact that $\partial_c \mathcal{E}^c_a \equiv 0$, we get that
\begin{equation}  %\label{SWM3}
\partial_a \Lambda^a \equiv i\, \left[A_a,\psi^a\right]\,, 
\end{equation} 
and, therefore, 
\begin{equation}  \label{SWM3}
\mathcal{E}^c_a Z^a \equiv \psi^c - i\,\Box^{-1}\partial^c \left[A_a,\psi^a\right]  \,.
\end{equation}

Provided that the definition (\ref{SWM2}) is invertible and that the homogeneous linear equation  admits only the trivial solution, then $\psi^c(A) = 0$ is equivalent to $\mathcal{E}^c_a Z^a = 0\,$. 

\begin{proposition} \label{P1}
Consider $Z_a$ a solution of $\mathcal{E}^c_a Z^a = 0\,$, and let $A_a(Z)$ and $Z_c$ be connected by the relation (\ref{SWM2}). If $A_a(Z)$ is ``small enough''\footnote{"small enough" refers to the fact that the definition of contract mapping must be met.} so that the linear equation $\,f^c - i\,\Box^{-1}\partial^c \left[A_a,f^a\right]=0$ has a unique solution, then $\,\psi_c\left(A(Z)\right) = 0\,$.
\end{proposition}

In any case, the definition (\ref{SWM2}) maps the nonlocal gauge field $A_a$ into the local field $Z_a\,$. What does the nonlocal gauge transformation $\delta  A_a = D_a \varepsilon\,$ become in terms of the local field $Z_a\,$? 

From (\ref{SWM1}), we have that
$$ i\,\delta \Lambda^a = \partial_c\left(\left[D^c\varepsilon,A^a\right] - \left[D^a\varepsilon,A^c\right]\right) + \left[D_c\varepsilon,F^{ca}\right]- i\left[A_c,\left[F^{ca},\varepsilon\right]\right] \,,$$
where (\ref{NC10}) has been included. Now, after a little algebra, we obtain that
$$ \left[D^c\varepsilon,A^a\right] - \left[D^a\varepsilon,A^c\right] = \partial^c\,\left[\varepsilon,A^a\right] - \partial^a\left[\varepsilon,A^c\right] - \left[\varepsilon, F^{ca}\right] $$
and that 
$$ \left[D_c\varepsilon,F^{ca}\right]- i\left[A_c,\left[F^{ca},\varepsilon\right]\right] = \partial_c\left[\varepsilon, F^{ca}\right] - \left[\varepsilon, \psi^a\right] \,,$$
which leads to
$$ i\,\Box^{-1}\,\delta \Lambda^a = \left[\varepsilon,A^a\right] - \partial^a \Box^{-1}\,\partial_c \left[\varepsilon,A^c\right] - \Box^{-1}\,\left[\varepsilon,\psi^a\right] \,.$$
Finally, combining the last equation with (\ref{SWM2}), we obtain
$$ \delta Z_a = D_a \varepsilon + i\,\left[A_a,\varepsilon\right] + i \,\partial_a \Box^{-1}\,\partial_c \left[\varepsilon,A^c\right] + i\,\Box^{-1}\,\left[\varepsilon,\psi_a\right]  \,$$
or
\begin{equation}  \label{SWM4}
\delta Z_a = \partial_a f + i\,\Box^{-1}\,\left[\varepsilon,\psi^a\right] \,, \qquad {\rm with} \qquad   f= \varepsilon + i \,\Box^{-1} \partial_c\left[\varepsilon, A^c\right] \,.
\end{equation}

If $A_a$ is a solution of $\psi^c$, then (\ref{SWM2}) maps it onto $Z_a$, which is a solution of the local field equations $\,\mathcal{E}^c_a Z^a=0\,$. Furthermore, it also maps the nonlocal gauge-transformed $\,A_a+ D_a\varepsilon\,$ onto the local gauge-transformed $\,Z_a + \partial_a f\,$. This achieves the goal, but only partially.


The Seiberg-Witten map \cite{Seiberg1999, Gomis2001_2} transforms the nonlocal, non-abelian gauge field $A_a$ into another field wherein the gauge is both commutative and local. The problem is solved  perturbatively up to the first order in $\theta^{ab}\,$, regardless of whether $A_a$ is a solution to the field equations.  Our mapping (\ref{SWM2}) achieves this goal, but only partially. Indeed, it establishes a one-to-one correspondence between solutions of the nonlocal field equations, $\psi_c=0$, and solutions of the local equations $\mathcal{E}^c_a Z^a=0$.  Moreover, it maps the non-abelian gauge-transformed of $A_a$ into the abelian gauge-transformed of $Z_a$, but only if $A_a$ is a solution of the field equations. This is why we have partially achieved our goal, the Seiberg-Witten map is achieved at the level of kinematic space, but not at the level of dynamical space. 

